Minotaur: Multi-Resource Blockchain Consensus

Resource-based consensus is the backbone of permissionless distributed ledger systems. The security of such protocols relies fundamentally on the level of resources actively engaged in the system. The variety of different resources (and related proof protocols, some times referred to as PoX in the literature) raises the fundamental question whether it is possible to utilize many of them in tandem and build multi-resource consensus protocols. The challenge in combining different resources is to achieve fungibility between them, in the sense that security would hold as long as the cumulative adversarial power across all resources is bounded. In this work, we put forth Minotaur, a multi-resource blockchain consensus protocol that combines proof-of-work (PoW) and proof-of-stake (PoS), and we prove it optimally fungible. At the core of our design, Minotaur operates in epochs while continuously sampling the active computational power to provide a fair exchange between the two resources, work and stake. Further, we demonstrate the ability of Minotaur to handle a higher degree of work fluctuation as compared to the Bitcoin blockchain; we also generalize Minotaur to any number of resources. We demonstrate the simplicity of Minotaur via implementing a full stack client in Rust (available open source). We use the client to test the robustness of Minotaur to variable mining power and combined work/stake attacks and demonstrate concrete empirical evidence towards the suitability of Minotaur to serve as the consensus layer of a real-world blockchain.

==> 0_abstract.tex <==
%%%
%%% OBSOLETE: abstract is inline in main.tex
%%%
\begin{abstract}
Resource-based consensus is the backbone of permissionless distributed ledger systems. 
%
The security of such protocols relies fundamentally on the level of resources actively engaged in the system. 
%
The variety of different resources (and related proof protocols, some times referred to as PoX in the literature) raises the fundamental question whether it is possible to utilize many of them in tandem and build {\em multi-resource} consensus protocols. The challenge in combining different resources is to achieve {\em fungibility} between them, in the sense that security would hold as long as the {\em  cumulative} adversarial power across all resources is bounded.  

In this work, we put forth \minotaurnosp, a multi-resource blockchain consensus protocol that combines proof of work (PoW) and proof-of-stake (PoS), and we prove it {\em  optimally} fungible. 
At the core of our design, \minotaur operates in epochs while continuously sampling the active computational power to provide a fair exchange between the two resources, work and stake. Further, we demonstrate the ability of \minotaur to handle a higher degree of work fluctuation as compared to \revreplace{the \bitcoin blockchain;}{previous PoW protocols such as the \bitcoin blockchain;} we also generalize \minotaur to any number of resources.  
  
We demonstrate the simplicity of \minotaur via implementing a full stack client in Rust (available open source~\cite{MinotaurcodeAnon}). We use the client to test the robustness of \minotaur to variable mining power and combined work/stake attacks and demonstrate concrete empirical evidence towards the suitability of \minotaur to serve as the consensus layer of a real-world blockchain. 
\end{abstract}


==> _introduction_backup.tex <==
\section{Introduction}



%para 1. Resource-based systems. (from Aggelos's PACM position paper). Resources include work1, work2, stake, space. 

%para 2. Grand question: how to bring different resources together. key challenge: how to normalize different resources so that they are exchangeable. 

%para 3. hybrid pow/pos approaches in the literature. simple ideas, but really dont work (point out their limitations). complex ideas (like the Zhou et al) also dont work. 
%There are some obvious improvements, but dont work for subtle reasons (cf. Section 4). 

%para 4. our main result: 4a: how we provide a new architecture and a resource normalization approach. Figure 1a: architecture depiction. 4b: performance is optimal and the best possible. (positive and converse). Figure 1b: performance depiction. 

%para 5. our result helps PoW chains in transient stage (bootstrapping). 

%para 6. our result helps PoS chains in transient stage (centralized allocation of stake).  

%para 7. experiments, implementation, simplicity. 

\noindent {\bf Resource-based Consensus}. Using the proof of possessing a resource as a mechanism to authorize participation in a consensus protocol is a central feature of the decentralized computing paradigm of blockchains. \bitcoin pioneered proof-of-work (PoW). The resulting resource wastage (large number of hash calculations) inspired the designs of proof-of-stake (PoS), proof-of-space (PoSp) and proof-of-elapsed-time (PoD).These different resources cover the  variegated and multidimensional forms of ``capital" that the participants bring.  Each  proof-of-X mechanism is interesting on their merit in appropriate settings (computation in PoW, memory and storage in PoSp and time/delay in PoD, tokens/capital in PoS). Further, the mechanisms trigger different incentives even within the same resource format; focusing on PoW for example, we see that  
 the hashcash algorithm \cite{} instantiated by the SHA256 function \cite{} implemented in \bitcoin  has been replaced by others, including  scrypt \cite{} and ethash \cite{}. Each of these different proof-of-X mechanisms have led to different, and isolated, blockchain ecosystems. 

\noindent {\bf Combining different resources}. Given the diversity of incentivization embodied by the different resources, it has been of great interest to combine their features in a single blockchain design (e.g., hybrid PoW-PoS permissioned blockchains). The key challenge to combining multiple resources is in determining the {\em exchange rate}:  adapting the exchange rate dynamically to the participation levels in each resource type, resulting in a truly {\em fungible}  notion of resource is a basic and fundamental  goal. By truly fungible, we mean that the security of the hybrid consensus protocol depends in {\em proportion} to the level of participation in each resource type. This property is made precise in the paper; below we give some examples of {\em nonfungible} hybrid consensus protocol designs. 

\noindent {\bf First order hybrid PoW/PoS protocols.} Given the basic importance of incorporating multiple resources in a single blockchain design, there are several  designs of  hybrid PoW/PoS protocols in the literature~\cite{KinNad12,BLMR14,FDKT+20,DCFZ18,karakostas2021securing}. These  protocols, however, are either heuristic (lacking a formal security  analysis)~\cite{KinNad12,BLMR14,DCFZ18}, or need unnecessary assumptions (e.g. honest majority in stake~\cite{FDKT+20,DCFZ18,karakostas2021securing} and static mining power~\cite{FDKT+20}).  
Indeed, with sufficient assumptions the problem of a hybrid protocol is trivially resolved. For instance, if we assume honest majority in stake (at all  time), we can use a committee chosen randomly from the pool of stakeholders to assist a PoW ledger by regularly issuing {\em checkpoints}~\cite{karakostas2021securing}. However, the security of this scheme is solely guaranteed by the stakeholders, and the trust is entirely supported by PoS (not from  PoW). 



\noindent {\bf Natural solutions}. %Point out some natural candidates and show they are vulnerable to subtle but fatal attacks. \xw{I wrote one natural solution in para 3.}
In fact, if we assume a static setting (where both the total mining power and total stake are fixed and known to the protocol designer), a simple solution is the following: PoW and PoS mining occur in parallel; whichever PoW or PoS mining succeeds first, it goes ahead and extends the longest chain. However, there does not appear to be any straightforward (or otherwise) approach   to extend this simple idea to the non-static setting; this is because,  we can no longer normalize the stake and work in the system when the total mining power is changing and unknown (\S~\ref{sec:base}).  Even a fungible combination of work (i.e., total amount of honest work is more than total Byzantine work) emanating from two different hash functions (thus allowing  two  PoW blockchains using the same longest-chain consensus protocol to co-exist) has been unsolved.
% TODO: 1. converse; 2. trivial solutions; 3. why this is hard. 

\noindent {\bf Minotaur Protocol.} In this paper we present \minotaurnosp, a blockchain protocol with proof of fungible work and stake. At its core, \minotaur is an epoch-based PoS longest chain protocol (e.g. Ouroboros family of protocols~\cite{kiayias2017ouroboros,david2018ouroboros,badertscher2018ouroboros}), but allows PoW mining to produce PoW blocks containing transactions. The PoW blocks will be selected by main chain blocks (i.e., PoS blocks) as payloads (or ``fruits''~\cite{pass2017fruitchains}). We define \textit{work stake} as a type of non-transferable tokens held by PoW miners as a ``proof of right" to propose PoS blocks in each epoch. Each epoch is assigned a certain amount of work stake that will be assigned to the PoW miners who succeed in mining PoW blocks; the work stake assigned to the respective miners is proportional to their work contribution \pv{what contribution? hash power?}\xw{actually it is the total difficulty of PoW blocks mined by the miner. But this is not well-defined here.} on the PoW blocks. PoS block production rights per epoch are then assigned by considering the {\it virtual stake}, that is the sum of actual stake (contributed by tokens) and work stake (contributed by PoW blocks). \xw{For instance, if Alice (who is a miner and a stakeholder at the same time) mines 20\% of the PoW blocks during epoch 1 and holds 10\% of the actual stake in the system by the end of epoch 1. Suppose the protocol sets the work stake to equal the actual stake, then Alice will control 15\% of the total virtual stake by the end of epoch 1. Later in epoch 3, Alice can generate PoS blocks with 15\% virtual stake as in a pure PoS protocol. Note that the spare epoch is for the main chain to stabilize and for preventing grinding on the work/actual stake. We highlight that the work stake is a key component in our design and it magically exchanges work into stake even in the dynamic setting.} Figure~\ref{fig:minotaur}  illustrates the protocol (a detailed description is in \S~\ref{sec:protocol}).

\noindent {\bf Minotaur security is optimal.} We show that \minotaur is secure when the sum of $\omega$ times the proportion of adversarial hash power ($\beta_w$) and $1-\omega$ times the proportion of the adversarial stake ($\beta_s$) is smaller than $1/2$, where $\omega \in [0,1]$ is a weighing parameter of PoW/PoS (see Figure~\ref{fig:pow_pos} for $\omega = 0.5$). Figure~\ref{fig:pow_pos} also compares the security guarantee of \minotaur and a couple of hybrid PoW/PoS protocols in the literature (the checkpointed ledger~\cite{karakostas2021securing} and the 2-hop blockchain~\cite{FDKT+20}). \pv{Write one sentence on the key technical idea behind the proof -- and point out how we merge the super-subtle variable difficulty mining rule in Bitcoin with the design of Minotaur} \xw{The challenge in our security analysis is to show a {\it fairness} guarantee in the work-stake conversion (e.g., a miner with 10\% mining power should gain 10\% work stake) under variable mining power. And this requires a new understanding of how to bound the evolution of mining difficulty in the system, which presents a significant barrier to surmount in our analysis.} We give a formal security analysis in Section~\ref{sec:proof}. One immediate consequence is that \minotaur can tolerate a 51\% mining adversary, as long as there is a supermajority in honest stake (and vice verse, a 51\% stake adversary). This kind of security guarantee is optimal, in the sense that otherwise the adversary will control the majority of ``resource'' in the system and an analogy of Nakamoto's private chain attack~\cite{nakamoto2008bitcoin} could break the security (formal and detailed proof in \S~\ref{sec:impos}). 



\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Minotaur.png}
        \caption{}
        \label{fig:minotaur}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/regions.png}
        \caption{}
        \label{fig:pow_pos}
    \end{subfigure}
    \caption{(a) Architecture of \minotaur consensus protocol. (b) Comparison of security regions achieved by different hybrid PoW/PoS protocols.}
\end{figure}

\noindent {\bf Implementation.} We have implemented a prototype of a \minotaur client in about 6000 lines of Rust code~\cite{Minotaurcode} and provide experimental results to evaluate the concrete performance of \minotaur under different scenarios. We also implemented a \bitcoin client as a benchmark. In particular, we show that \minotaur can survive more drastic variations of network hash power, while \bitcoin is no longer live under the same scenario. We also evaluate practical security concerns, like selfish mining and spamming, on our \minotaur client. Our implementation shows that \minotaur performs well even under these attacks, and makes a stronger case for the practical viability and robustness of the system. More details on the implementation and the experiments can be found in Section~\ref{sec:exp}.

\noindent {\bf Application and discussion.} We point out that \minotaur provides a secure and efficient method to bootstrap PoW blockchains. In general, it is more challenging to securely launch PoW blockchains, as a new blockchain would presumably start off with a relatively smaller total computation power and be vulnerable to the so-called ``51\% attacks''. On the other hand, PoS blockchains are easy to launch with existing techniques, such as proof-of-burn~\cite{karantias2020proof}, initial coin offering~\cite{li2018initial} and airdrop~\cite{airdrop}. Therefore, \minotaur can be launched as a pure PoS blockchain and later transit into a pure PoW blockchain by smoothly changing the weighing parameter $\omega$. In this paper, we also discuss how to bootstrap \minotaur in a purely decentralized manner. See all these in Section~\ref{sec:discuss}.


\noindent {\bf Related work.}
The idea of hybrid PoW/PoS block production was first mentioned in~\cite{KinNad12}. A first concrete construction was given in~\cite{BLMR14} under the label `proof of activity', but without giving a rigorous security analysis. Their block-production mechanism essentially extends standard \bitcoin mining by having the mined block implicitly elect a set of stake holders that are required to sign the block in order to validate it.

A similar construction was proposed in~\cite{FDKT+20} and proven secure under a majority of adversarial hashing power---however, their security proof still implies an honest majority of stake. In particular, and contrary to their initial claims, the protocol is not proven secure under the condition that \emph{any} minority of the combined resources is controlled by the adversary.

The work of~\cite{FDKT+20} was extended in~\cite{DCFZ18}, to adapt to dynamic participation of both, hashing power and stake, and in~\cite{TNDF+18}, to combine PoW with multiple resources (rather than just PoS)---both works lack a rigorous security analysis.

\cite{CXGL+18} were the first to explicitly motivate PoW/PoS hybrid block production by the goal of protecting early-stage PoW systems against initial periods of adversarial dominance in hashing power. They propose to start the system with hybrid block production (where each resource contributes to a certain fraction of the blocks) and then slowly fade out the stake contribution to eventually turn the system into pure proof of work. Also this protocol is not proven secure.

\ignore{
The 2-hop blockchain~\cite{FDKT+20} is also a hybrid PoW/PoS protocol, which aims to survive the 51\% mining attack. In a 2-hop blockchain, there are two coupled blockchains, one  based a PoW mechanism and another using a PoS-based approach, and these two blockchains are extended alternately. However, the protocol is only designed for the static computing power and stake setting, which makes it unpractical. In addition, \minotaur is more flexible as weighing PoW and PoS can be supported.  
}


==> appz_revision.tex <==
\clearpage
\section*{Revision Notes}

This section restates the change requests by the reviewers followed by the main part of the paper
wherein the respective changes are marked.

The paper changes are marked with four different color codes as follows, where the initial number is the change number and (reference) refers to the respective reviewer request(s):\footnote{If there is no (reference) then the change does not directly relate to one particular request.}

\medskip

\revhighlight[(reference)]{
 This text is original and should already respond to the request.
}

\medskip

\revadd[(reference)]{
 This text was added in contrast to the original submission.
}

\medskip

\revdelete[(reference)]{
 This text was removed in contrast to the original submission.
}

\medskip

\revreplace[(reference)]{ %
 This text was original and is now deleted.
} %
{
 This text replaces the deleted original text.
}

\medskip


Here is a summary of our major revisions. 

\begin{itemize}
    \item As suggested by the reviewers, we have explicitly clarified the motivation to combine PoW and PoS in~\S\ref{sec:intro}.
    \item We have acknowledged the downsides and limitations of combining PoW and PoS in~\S\ref{sec:discuss}.
    \item We have added comparisons with related works, including 1) arguing why other approaches are insufficient to handle 51\% attack during launch; 2) performance comparisons with the state-of-the-art PoW/PoS protocols.
    \item We have implemented \fruitchains and Ouroboros clients as benchmarks in our experiments.
    \item We have added private chain attack experiments on \minotaurnosp/\bitcoinnosp/Ouroboros to provide empirical evidence that \minotaur is better than pure PoW or PoS.
    \item We have added \fruitchains as a baseline in variable difficulty experiment and selfish mining attack experiment. The results showed that \minotaur is better than \fruitchains in both experiments.
\end{itemize}

Below we also describe our specific responses to the revision requests with pointers to the paper. Our responses are marked in {\color{magenta} color} to easily distinguish them from the reviewer comments. 

\subsection*{Requests in program-chair e-mail}
Based on the rebuttal, here are some of the suggested changes:
\begin{enumerate}
    \item\label{req:motivation} Explicitly clarify the introduction's motivation to combine PoW and PoS. {\color{magenta} (See Changes~\ref{ans:motivation} and~\ref{ans:motivation:2})}
    \item\label{req:limitations} Also, acknowledge the downsides and limitations of combining PoW and PoS. 
    {\color{magenta} (See Change~\ref{ans:limitations})}
    \item\label{req:51} 51\% attack during launch: Argue why other approaches are insufficient to handle this scenario. 
    {\color{magenta} (See Changes~\ref{ans:51} and~\ref{ans:51:2})}
    \item\label{req:revamp} Revamp the experiments to empirically convince why a hybrid of PoW and PoS is better than pure PoW or PoS. 
    {\color{magenta}  (See Changes~\ref{ans:privatechain} where we illustrate this point by designing and executing a new set of experiments). }
\end{enumerate}

\subsection*{Requests by reviewer A}
Concerns to be addressed during the revision/shepherding:
\begin{enumerate}[resume]
\item\label{req:incremental} Since the paper presents incremental research over previous similar work, a better comparison to related work and describing what is the novelty of \minotaur protocol and methods is needed. {\color{magenta}  (See comment below)}
\item\label{req:comparison} Also, it is good to add some performance comparisons to justify the benefits. {\color{magenta} (See Change~\ref{ans:comparison} and comment below.)}
\end{enumerate}

{\color{magenta} 
\paragraph{Response to Request~(\ref{req:incremental}).}
We disagree with the assessment that we present ``incremental research'':  Blockchain protocols are complex systems and research advances typically share structural characteristics with previous protocols to achieve novel properties (e.g., Ouroboros~\cite{kiayias2017ouroboros} uses the same longest-chain structure as \bitcoin but for PoS, \fruitchains~\cite{pass2017fruitchains} uses the 2-for-1-PoW technique of~\cite{GKL2015}  but for fairness, etc). Similarly, the \minotaur design may look incremental over previous work — the novelty though is that fungibility in multi-resource blockchains was never achieved before and several other similar designs (see \S\ref{sec:intro}) fail to be secure. Recognizing the subtleties in coming up with a truly fungible and secure hybrid PoW/PoS design along with a careful security analysis are our main contributions.
}

{\color{magenta} 
\paragraph{Response to Request~(\ref{req:comparison}).}
Note also that the motivation for \minotaur are different security guarantees, and not increased performance. We clarified the motivation in Changes~\ref{ans:motivation} and~\ref{ans:motivation:2}.
}

\subsection*{Requests by reviewer B}
Questions for authors’ response:
\begin{enumerate}[resume]
\item\label{req:b:motivation} Kindly clarify the motivation behind combining PoW and PoS. {\color{magenta}  (See Request~\ref{req:motivation}) }
\item Briefly describe an experimental setup that would empirically convince why a hybrid of PoW and PoS is better than pure PoW or PoS. {\color{magenta}  (See Request~\ref{req:revamp})}
\end{enumerate}

\subsection*{Requests by reviewer C}
Weaknesses / Reasons to reject:
\begin{enumerate}[resume]
\item\label{req:initialstake} It is overpromised to say \minotaur is fungible and does not require an honest majority in stake distribution. The approaches to relaxing this assumption are only mentioned in the discussion. If indeed this can be released, one needs to reproduce the security proofs, which currently mainly come from Ouroboros works. For example, Theorem 6.4 is not immediate from Theorem 3 in ``Ouroboros Praos'' because there, the distribution is on actual stakes held by the adversary and Theorem 6.4 considers virtual stakes defined in this work. If the initial stake distribution does not guarantee an honest majority, this needs to be proved. {\color{magenta}  (See Change~\ref{ans:initialstake}) }
% XW: We only assume an honest majority in the initial stake distribution. Relaxing this assumption needs to alter the protocol, not just the proof. We  
\item\label{req:virtualstake} The proof that ``honest majority in virtual stake'' implies ``security for PoS chain'' is not explicitly given. This is an important part of generalizing theorems in a single epoch to longer periods. The authors point to proofs for Theorem 5.3 in ``Ouroboros'', which is for stakes instead of virtual stakes calculated in this work. It's not obvious that they should follow the same arguments unless an honest majority in virtual stakes implies an honest majority in pure stakes. But the latter brings doubts to the assumption that it is only required to have an honest majority in initial stake distribution. {\color{magenta}  (See Change~\ref{ans:virtualstake}) }
% XW: The main-chain blocks are scheduled according to the virtual/actual stake distribution in Minotaur/Ouroboros respectively. This is why we can use the machinery of Ouroboros proof directly.
\item\label{req:qualityandgrowth} The security guarantees are weaker than other works, e.g., Ouroboros Praos. Chain Growth property is not discussed, which affects liveness, thus affecting the three major theorems, Theorem 6.1-6.3. Explaining why leaving out chain growth or why existential chain quality and common prefix implies liveness is necessary. Also, existential chain quality is weaker than chain quality, which specifies the upper bound for the portion of adversary-controlled blocks in some snippet of a chain with length $\geq k$. Existential chain quality only needs the honest party to control at least 1 block. {\color{magenta}  (See Change~\ref{ans:qualityandgrowth} and comment below) }
% XW: The goal of the security proof is to show persistence and liveness of Minotaur, which are defined the same as in Ouroboros Praos. Chain growth, (existential) chain quality and common prefix are just intermediate properties. We will justify why existential chain quality and common prefix suffice to imply liveness in the proof of Theorem 6.9.
\item\label{req:adaptivity} Besides, this work claims to allow adaptive adversary, which is never discussed beyond the statement that it is hard. It was not immediately clear how adaptive security of Ouroboros can result in adaptive security here. {\color{magenta}  (See Change~\ref{ans:adaptivity}) }
% XW: We only allow adaptive corruption of miners, but not stakers. This means both the number of honest miners and the number of corrupted miners in each slot are chosen by the adversary. Therefore, the PoW mining processes in each slot are no longer independent and this is handled by the martingale argument in our proof. 
\end{enumerate}

Constructive comments for author:
\begin{enumerate}[resume]
\item\label{req:qualityandgrowth:2} If possible, using chain quality instead of existential chain quality can produce stronger results. {\color{magenta} (See Request~\ref{req:qualityandgrowth}) }
% XW: Existential chain quality, together with common prefix, suffices to imply liveness.

\item\label{req:lemma6.5} In the proof for Lemma 6.5, ``by the existential CQ, the tip of ... has timestamp'' does not seem to make sense. Chain growth can tell about timestamps but existential CQ only tells one that in a long enough chain snippet, there's at least an honest block. {\color{magenta} (See comment below). }
% XW: By the existential CQ, there is at least one honest block in the chain C^k with a timestamp in the interval [r_0-2k,r_0-k]. And since the timestamps must be increasing in a chain, therefore the tip of C^k has timestamp at least r_0-2k

\item\label{req:c:motivation} Stating the motivations for this work, e.g., to argue what including an extra PoW chain brings, especially what PoS fails and this hybrid approach picks up, is important. Right now, the security guarantees seem to be weaker and I do not see gains from having the extra PoW chain as endorser while the consensus is essentially PoS. Maybe it adds unnecessary complexity? {\color{magenta} (See our response to Request~\ref{req:motivation} and Request~\ref{req:revamp})}

\item\label{req:fccomparison} Besides, since the consensus is essentially PoS, comparing the protocol with \bitcoin on selfish mining resistance does not make much sense. Because selfish mining means to hold discovered blocks to waste others' mining power. {\color{magenta} (This is not true; Nakamoto-style PoS protocols are also susceptible to selfish-mining type of attacks which reduce Chain Quality in a similar manner as in \bitcoin. It is a good point though to extend comparison appropriately and we also included \fruitchains in our comparison. See Changes~\ref{ans:fccomparison},~\ref{ans:fccomparison:2}, and~~\ref{ans:fccomparison:3} and Table~\ref{tab:selfish_mining})
% XW: The goal of selfish mining is to reduce chain quality and gain more block reward. It applies to PoS as well.
}
\end{enumerate}

\paragraph{Additional response to Request~(\ref{req:qualityandgrowth}).}
{\color{magenta} 
The goal of the security proof is to show persistence and liveness of \minotaurnosp, which are defined the same as in Ouroboros Praos~\cite{david2018ouroboros}. Chain growth, (existential) chain quality and common prefix are just intermediate properties. Existential chain quality, together with common prefix, suffices to imply liveness (see Change~\ref{ans:qualityandgrowth}). }


\paragraph{Additional response to Request~(\ref{req:lemma6.5}).}
{\color{magenta} 
By the existential CQ, there is at least one honest block in the chain $\mathcal{C}^{\lceil \kappa}$ with a timestamp in the interval $[r_0-2\kappa,r_0-\kappa]$. And since the timestamps must be increasing in a chain, therefore the tip of $\mathcal{C}^{\lceil \kappa}$ has timestamp at least $r_0-2\kappa$.}

%%%%%%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%%%%%%%%%
























\ignore{
\subsection{old}

\noindent \textbf{TODO: by argument}
\begin{enumerate}[label=\Alph*]
\item\label{req:comparison} Comparison to previous work. \mf{done.
    In `release note': defend why the work is not incremental.}
    \item\label{req:perf_comparison} Performance comparisons to state-of-the-art protocols. \mf{pending.}
    \item\label{req:51} 51\% attack during launch: Argue why other approaches are insufficient to handle this scenario. \mf{done.}
\end{enumerate}

\noindent \textbf{TODO: by experiment}
\begin{itemize}
    \item Add \fruitchains as Baseline in variable difficulty experiment and selfish mining attack \xw{Done.}
    \item Revamp the experiments to empirically convince why a hybrid of PoW and PoS is better than pure PoW or PoS.
\end{itemize}




\subsection*{Comments by reviewer A}

\noindent {\bf Weaknesses/Reasons to reject}
While the theory is strong, the paper falls short of convincing why this protocol is useful in practice. Why does a real system need to use multiple resources together? Why do authors assume a dynamic environment between the resources? \re{Relying on a single resource makes the consensus protocol susceptible to sudden large fluctuations in the availability of the underlying resource. Examples: (1) in PoW there can be a sudden influx of hashing power, e.g., when a new PoW blockchain is launched, or a sudden loss of hashing power when many miners depart (e.g., due to a mining ban), (2) in PoS there can be a sudden drop of coin value (e.g., during a stock market crash). Such fluctuations can be adversarially exploited. Fungible multi-resource consensus like \minotaur results in better resilience and predictability protecting the system against sudden unilateral fluctuations in any single one of the underlying resources. This is now highlighted in \S\ref{sec:intro}.}

The paper is incremental research over previous similar work and mainly adds security proof to similar techniques. It is not easy to distinguish the novelty of the \minotaur protocol from the previous work.
\re{We disagree with the assessment that we present ``incremental research'':  Blockchain protocols are complex systems and research advances typically share structural characteristics with previous protocols to achieve novel properties (e.g., Ouroboros~\cite{kiayias2017ouroboros} uses the same longest-chain structure as \bitcoin but for PoS, \fruitchains~\cite{pass2017fruitchains} uses the 2-for-1-PoW technique of~\cite{GKL2015}  but for fairness, etc). Similarly, the \minotaur design may look incremental over previous work — the novelty though is that fungibility in multi-resource blockchains was never achieved before and several other similar designs (see \S\ref{sec:intro} and \S\ref{sec:base}) fail to be secure. Recognizing the subtleties in coming up with a truly fungible and secure hybrid PoW/PoS design along with a careful security analysis are our main contributions. This is now highlighted in the paper.}

The paper does not show a comprehensive evaluation of the new protocol compared to the state of the art in terms of performance and speed.
\re{The motivation for \minotaur are different security guarantees, and not increased performance. We added performance comparison with state-of-the-art protocols.}

\noindent {\bf Constructive comments for author}
The proposed protocol is simple and easy to follow and understand. The proofs are readable and nicely written which is a big plus. The theory is strong and it is interesting to read how multiple resources can be used together in a consensus system even when the environment is dynamic. \re{Thanks for the comments!}

\noindent {\bf Some overall comments to improve the paper:}

To address the issue of why this protocol is useful in practice, I suggest the authors spend more time on motivating this work and try to show why this is an interesting problem to solve.

The paper does not show a comprehensive evaluation result of the new protocol compared to the state of the art in terms of performance and speed. How much does the fact that the protocol is working in a multi-resource setting change the throughput of the system? \re{Thanks for these comments. They are now addressed as mentioned above.}

\noindent {\bf Detailed comments:}

Page 1. Many PoS protocols are not permissionless unlike what is suggested by authors in the first paragraph of the introduction.
\re{The focus of this paper is on (truly) permissionless PoS systems that should support dynamic stake.}

Page 1. Taking control of different resources does not have the same cost for the adversary. I suggest the authors create a resource-competitive framework and dynamic for analyzing the multi-resource consensus protocol. \re{Thanks for the suggestion. However, due to the time/space limit, we decided to defer such framework and analysis to the future work.}

Page 2. The paragraph that describes the \minotaur Protocol is not clear. Specifically, the reader should go back to read three related works to understand the protocol. For example, please add a simple description of fairness mechanisms.
\re{More details on the related protocols can be found in Appendix~\ref{app:ouroboros}. A pointer is now added in the main text. The fairness mechanism is simply to assign work state proportionally to work blocks as described in our protocol.}

Page 4, 2.3: need space after ``bound:''.
\re{Fixed. Thanks for catching it.}

\noindent {\bf Concerns to be addressed during the revision/shepherding}
Since the paper presents incremental research over previous similar work, a better comparison to related work and describing what is the novelty of \minotaur protocol and methods is needed. Also, it is good to add some performance comparisons to justify the benefits. \re{Thanks for these comments. They are now addressed as mentioned above.}

\subsection*{Comments by reviewer B}

\noindent {\bf Weaknesses/Reasons to reject}

\begin{itemize}
    \item Motivation to diversify the Sybil resistance mechanism not articulated clearly
    \item Baseline comparison in the experimental evaluation 
\end{itemize}

\noindent {\bf Constructive comments for author} 

Motivation: Paper identifies the following motivations to combine PoS and PoW:
\begin{enumerate}
    \item Diversification of the resources
    \item Different incentives structures across PoXs/within each PoX
    \item Different PoX mechanisms lead to isolated ecosystems
    \item Protecting PoW blockchains from ``51\% attack'' during the launch
\end{enumerate}

It would help the readers if the paper could clarify why combining PoW and PoS is the solution for any of these reasons.
\begin{enumerate}
    \item Diversification of the resources: PoW is truly permissionless because protocol and nodes do not know the exact number of the participants, and there is no way to authenticate participants. Unfortunately, this comes with the price of a large energy footprint (as acknowledged in the paper). However, in the \minotaur protocol, PoW miners must include their PK to convert their mining efforts as virtual stakes. If the miners do not include their PKs, the protocol collapses to PoS without fungibility between PoS and PoW. Thus, having PK in PoW inherits the downsides of PoW without its advantages. On the contrary, the protocol loses its fungibility by not including PK in PoW. Potentially PoS and other PoX$\setminus$PoW can be combined together. However, explaining the reason to do this would substantially help the readers. \re{Thanks for the comments. We now explicitly clarify the motivation to combine PoW and PoS in \S\ref{sec:intro} and also acknowledge the downsides and limitations of combining PoW and PoS in \S\ref{sec:discuss}.}
    \item Different incentives structures across PoXs/within each PoX: PoW, as used in \bitcoin, is not incentive compatible. SHA256 is not ASIC resistant, thus centralizing the mining power. Whereas scrypt and ethash are ASIC resistant and easy to verify, thus mitigating centralized mining pools. Why resources coming from centralized mining pools should be combined with other resources in a decentralized system?
    \re{After the combination, the protocol may be resistant to attacks from an even larger centralized mining pool, e.g. one with 70\% of the SHA256 hash power.}
    \item Different PoX mechanisms lead to isolated ecosystems: It is unclear why approaches such as bridges/cross chains are not enough for blockchain interoperability. \re{}
    \item Protecting PoW blockchains from ``51\% attack'' during the launch: It is evident that \minotaur can start as pure PoS and gradually transition to pure PoW. However, it is not clear how other strawmen/simpler approaches fall short. \re{}
\end{enumerate}

Baseline comparison: The choice for baseline comparison in Section 7 has to be justified. Currently, the paper acknowledges the fairness limitations of \bitcoin and yet compares the performance \minotaur with \bitcoinnosp. Thus, Table 2 comes as no surprise. It is evident that \fruitchains is the most appropriate choice for baseline comparison in Section 7.3, as \minotaur aims to improve upon it. \re{Thanks for the suggestion. We now add comparison with \fruitchains under the selfish mining attack. Notice that \minotaur will still outperform \fruitchains when the fraction of adversarial mining power $> 0.5$.}

It is impressive that \minotaur can tolerate fluctuations in the mining power. However, the current experimental section does seem to justify why it is realistic to assume that the \bitcoin mining power could drop exponentially. In contrast, the mining power in \bitcoin has gone up exponentially since its inception and current approaches to calibrate difficulty seem to have worked out for \bitcoin. \re{Other PoW blockchains that use the same difficulty adjustment rule may experience such drop. For example, ETC dropped from 19 TH/s to 1.5 TH/s in 7 months period \url{https://2miners.com/etc-network-hashrate}, but more impressively ERGO dropped from 23.65 to 0.5 TH/s in just 2 weeks' time \url{https://2miners.com/erg-network-hashrate}. This is now made clear in \S\ref{sec:fluctuation analysis}.}

At a high level, the experimental section does not empirically convince why a hybrid of PoW and PoS is better than pure PoW or PoS. \re{Thanks for the comment. We added a private chain attack experiment in \S\ref{sec:exp} to empirically demonstrate this.}

\noindent {\bf Conclusion} Overall I believe that the protocol works, however, the reasons to combine PoW and PoS are not clear from Section 1 or 7.

\noindent {\bf Questions for authors’ response}
\begin{itemize}
    \item Kindly clarify the motivation behind combining PoW and PoS
    \item Briefly describe an experimental setup that would empirically convince why a hybrid of PoW and PoS is better than pure PoW or PoS
\end{itemize}
\re{Thanks for these comments. They are now addressed as mentioned above.}


\subsection*{Comments by reviewer C}

\noindent {\bf Weaknesses/Reasons to reject}

\begin{enumerate}
    \item It is overpromised to say \minotaur is fungible and does not require an honest majority in stake distribution. The approaches to relaxing this assumption are only mentioned in the discussion. If indeed this can be released, one needs to reproduce the security proofs, which currently mainly come from Ouroboros works. For example, Theorem 6.4 is not immediate from Theorem 3 in ``Ouroboros Praos'' because there, the distribution is on actual stakes held by the adversary and Theorem 6.4 considers virtual stakes defined in this work. If the initial stake distribution does not guarantee an honest majority, this needs to be proved. \re{We only assume an honest majority in the initial stake distribution and we believe this is reasonable. Relaxing this assumption needs to alter the protocol, not just the proof. We defer this to the future work. This is now made clear in \S\ref{sec:discuss}.}
    \item The proof that ``honest majority in virtual stake'' implies ``security for PoS chain'' is not explicitly given. This is an important part of generalizing theorems in a single epoch to longer periods. The authors point to proofs for Theorem 5.3 in ``Ouroboros'', which is for stakes instead of virtual stakes calculated in this work. It's not obvious that they should follow the same arguments unless an honest majority in virtual stakes implies an honest majority in pure stakes. But the latter brings doubts to the assumption that it is only required to have an honest majority in initial stake distribution. \re{The main-chain blocks are scheduled according to the virtual/actual stake distribution in \minotaurnosp/Ouroboros respectively. The Ouroboros analysis thus directly translates by replacing their actual stake by virtual stake. This is now made clear in \S\ref{sec:proof}.}
    \item The security guarantees are weaker than other works, e.g., Ouroboros Praos. Chain Growth property is not discussed, which affects liveness, thus affecting the three major theorems, Theorem 6.1-6.3. Explaining why leaving out chain growth or why existential chain quality and common prefix implies liveness is necessary. Also, existential chain quality is weaker than chain quality, which specifies the upper bound for the portion of adversary-controlled blocks in some snippet of a chain with length $\geq k$. Existential chain quality only needs the honest party to control at least 1 block. \re{The goal of the security proof is to show persistence and liveness of \minotaurnosp, which are defined the same as in Ouroboros Praos. Chain growth, (existential) chain quality and common prefix are just intermediate properties. We now justify why existential chain quality and common prefix suffice to imply liveness in the proof of Theorem~\ref{thm:re_main}.}
    \item Besides, this work claims to allow adaptive adversary, which is never discussed beyond the statement that it is hard. It was not immediately clear how adaptive security of Ouroboros can result in adaptive security here. \re{We allow instantaneously adaptive corruption on miners. This means both the number of honest miners and the number of corrupted miners in each slot are chosen by the adversary. Therefore, the PoW mining processes in each slot are no longer independent and this is handled by the martingale argument in our proof. For stakers, the adversary is only ‘moderately’ adaptive (participant corruption only takes effect after a certain delay), just like in Ouroboros classic. This is now made clear in \S\ref{sec:prelim}.}
\end{enumerate}

\noindent {\bf Constructive comments for author}

\begin{enumerate}
    \item If possible, using chain quality instead of existential chain quality can produce stronger results. \re{Existential chain quality, together with common prefix, suffices to imply liveness. This is now justified in the proof of Theorem~\ref{thm:re_main}.}
    \item In the proof for Lemma 6.5, ``by the existential CQ, the tip of ... has timestamp'' does not seem to make sense. Chain growth can tell about timestamps but existential CQ only tells one that in a long enough chain snippet, there's at least an honest block. \re{By the existential CQ, there is at least one honest block in the chain $\mathcal{C}^{\lceil \kappa}$ with a timestamp in the interval $[r_0-2\kappa,r_0-\kappa]$. And since the timestamps must be increasing in a chain, therefore the tip of $\mathcal{C}^{\lceil \kappa}$ has timestamp at least $r_0-2\kappa$.}
    \item Stating the motivations for this work, e.g., to argue what including an extra PoW chain brings, especially what PoS fails and this hybrid approach picks up, is important. Right now, the security guarantees seem to be weaker and I do not see gains from having the extra PoW chain as endorser while the consensus is essentially PoS. Maybe it adds unnecessary complexity? \re{The motivation for this work is now explicitly stated in \S\ref{sec:intro}.} 
    \item Besides, since the consensus is essentially PoS, comparing the protocol with \bitcoin on selfish mining resistance does not make much sense. Because selfish mining means to hold discovered blocks to waste others' mining power. \re{The goal of selfish mining is to reduce chain quality and gain more block reward. It applies to PoS as well.}
\end{enumerate}


\noindent {\bf Misc:}

\begin{enumerate}
    \item The abstract does not seem to reflect what is achieved in this work. Several statements mentioned are only touched on in the last section of the brief discussion. \re{It seems the only statement is ``we also generalize \minotaur to any number of resources''.}
    \item The preliminaries can be shortened to make room for proofs original to this work. \re{}
    \item  The optimality of \minotaur seems to be weird because in Figure 1(b), checkpointed ledger seems to outperform when adversary hashing power is over 50\% (maybe because it always has stakeholders to assist in finalizing blocks). More explanation or some adjustment for this figure can be helpful in this aspect. \re{By optimality, we mean the region below the curve in Figure~\ref{fig:pow_pos} cannot be enlarged any more. Therefore, the checkpointed ledger is also optimal, but that region can also be achieved by \minotaur with $\omega= 0$. This is now justified in \S\ref{sec:impos}.}
    \item Fig 3 proves the security for the PoS and PoW combination. First, PoS provides CP+Existential CQ and PoW provides fairness, then with additional assumption, you have an honest majority in virtual stake. If one replaces PoS and/or PoW with other resources, does the proof still follow immediately? \re{In generalized version of \minotaur (\S\ref{sec:discuss}), PoW blocks are replaced by ‘resource blocks’ while PoS blocks (main-chain blocks) remain. Note that stake is not required to be one of the resources, as we can assign zero weight to the actual stake when computing the virtual stake. For the proof, the PoW fairness argument will be replaced by fairness with respect to the other resources. This is now made clear in \S\ref{sec:discuss}.}
\end{enumerate}




}
